Automated Code Repair for C/C++ Static Analysis Alerts

(Note: This work is a preprint.) Static analysis (SA) tools produce many diagnostic alerts indicating that source code in C or C++ may be defective and potentially vulnerable to security exploits. Many of these alerts are false positives. Identifying the true-positive alerts and repairing the defects in the associated code are huge efforts that automated program repair (APR) tools can help with. Our experience showed us that APR can reduce the number of SA alerts significantly and reduce the manual effort of analysts to review code. This engineering experience paper details the application of design, development, and performance testing to an APR tool we built that repairs C/C++ code associated with 3 categories of alerts produced by multiple SA tools. Its repairs are simple and local. Furthermore, our findings convinced the maintainers of the CERT Coding Standards to re-assess and update the metrics used to assess when violations of guidelines are detectable or repairable. We discuss engineering design choices made to support goals of trustworthiness and acceptability to developers. Our APR tool repaired 8718 out of 9234 alerts produced by one SA tool on one codebase. It can repair 3 flaw categories. For 2 flaw categories, 2 SA tools, and 2 codebases, our tool repaired or dismissed as false positives over 80% of alerts, on average. Tests showed repairs did not appreciably degrade the performance of the code or cause new alerts to appear (with the possible exception of sqlite3.c). This paper describes unique contributions that include a new empirical analysis of SA data, our selection method for flaw categories to repair, publication of our APR tool, and a dataset of SA alerts from open-source SA tools run on open-source codebases. It discusses positive and negative results and lessons learned.

==> mathmode-spacing.tex <==
% Source: http://tex.stackexchange.com/a/129454
% Adjusts spacing between letters in math mode for multiple-letter identifiers.

\usepackage{etexcmds}

\makeatletter
\newtoks\m@toks@math
\newtoks\m@toks@text

\edef\m@tmp@restore{%
  \lccode\number`\X=\the\lccode`\X\relax
  \lccode\number`\~=\the\lccode`\~\relax
}

\newcommand*{\m@activate}{}
\newcommand*{\m@check@letter}{}
\newcommand*{\m@check@fi}{}

\newif\ifm@single

\let\m@start\relax
\def\m@loop{%
  \lccode`\X=\count@
  \lccode`\~=\count@
  \lowercase{%
    \expandafter\mathchardef\csname m@code@X\endcsname=\mathcode\count@
    \edef\m@activate{%
      \etex@unexpanded\expandafter{\m@activate}%
      \mathcode\the\count@="8000\relax
      \def\noexpand~{\m@start\csname m@code@X\endcsname X}%
    }%
    \g@addto@macro\m@check@letter{%
      \ifx\@let@token X\else
    }%
  }%
  \g@addto@macro\m@check@fi{\fi}%
  \advance\count@\@ne
}
% A-Z
\count@=`\A\relax
\@whilenum\count@<\numexpr`\Z+1\relax\do{\m@loop}
% a-z
\count@=`\a\relax
\@whilenum\count@<\numexpr`\z+1\relax\do{\m@loop}

\newcommand*{\m@start}[2]{%
  \bgroup
  \m@toks@math{#1}%
  \m@toks@text{#2}%
  \m@singletrue
  \futurelet\@let@token\m@check
}
\edef\m@check{%
  \etex@unexpanded{%
    \let\m@next\m@add
    \ifx\@let@token\space
      \let\m@next\m@finish
    \else
      \ifx\@let@token\egroup
        \let\m@next\m@finish
      \else
  }%
  \etex@unexpanded\expandafter{%
        \m@check@letter
  }%
  \etex@unexpanded{%
          \let\m@next\m@finish
  }%
  \etex@unexpanded\expandafter{%
        \m@check@fi
  }%
  \etex@unexpanded{%
      \fi
    \fi
    \m@next
  }%
}

\newcommand*{\m@add}[1]{%
  \m@singlefalse
  \m@toks@math\expandafter{%
    \the\expandafter\m@toks@math
    \csname m@code@#1\endcsname
  }%
  \m@toks@text\expandafter{%
    \the\m@toks@text
    #1%
  }%
  \futurelet\@let@token\m@check
}

\newcommand*{\m@finish}{%
  \ifm@single
    \expandafter\mprintsingle\expandafter{%
      \the\expandafter\m@toks@math\expandafter
    }\expandafter{%
      \the\expandafter\m@toks@text\expandafter
    }%
  \else
    \expandafter\mprintmulti\expandafter{%
      \the\expandafter\m@toks@math\expandafter
    }\expandafter{%
      \the\expandafter\m@toks@text\expandafter
    }%
  \fi
  \egroup
}
\let\mprintsingle\@firstoftwo
\let\mprintmulti\@firstoftwo

\everymath{\m@activate}
\everydisplay{\m@activate}

\m@tmp@restore
\makeatother

\renewcommand*{\mprintsingle}[2]{{#1}}%
\renewcommand*{\mprintmulti}[2]{\mathit{#1}}%

